Wave splitting of Maxwell's equations with anisotropic heterogeneous constitutive relations

The equations for the electromagnetic field in an anisotropic media are written in a form containing only the transverse field components relative to a half plane boundary. The operator corresponding to this formulation is the electromagnetic system's matrix. A constructive proof of the existence of directional wave-field decomposition with respect to the normal of the boundary is presented. In the process of defining the wave-field decomposition (wave-splitting), the resolvent set of the time-Laplace representation of the system's matrix is analyzed. This set is shown to contain a strip around the imaginary axis. We construct a splitting matrix as a Dunford-Taylor type integral over the resolvent of the unbounded operator defined by the electromagnetic system's matrix. The splitting matrix commutes with the system's matrix and the decomposition is obtained via a generalized eigenvalue-eigenvector procedure. The decomposition is expressed in terms of components of the splitting matrix. The constructive solution to the question on the existence of a decomposition also generates an impedance mapping solution to an algebraic Riccati operator equation. This solution is the electromagnetic generalization in an anisotropic media of a Dirichlet-to-Neumann map.

==> now_macro.tex <==
\newcommand{\signature}{B. L. G. Jonsson}


\makeatletter
% catches author and title for the headers, must be before \maketitle
% that clears the
% variables \@author and \@title

\def\catchNameTitle{
\global\let\Author\@author \global\let\Title\@title }

% creates a string with the time now.
\def\timenow{%
  \@tempcnta=\time \divide\@tempcnta by 60 \number\@tempcnta:\multiply
  \@tempcnta by 60 \@tempcntb=\time \advance\@tempcntb by -\@tempcnta
  \ifnum\@tempcntb <10 0\number\@tempcntb\else\number\@tempcntb\fi}

% creates a string with todays date Swedish version
\def\TODAY{\number\year-\ifcase\month\or 01\or 02\or 03\or 04\or 05\or
    06\or 07\or 08\or 09\or 10\or 11\or 12\fi-\ifnum\day<10 0\number\day\else \number\day\fi}

% substitute for markboth or simular commands sets the page with #1
%to #4 one in each corner on every page

\newcommand{\MarkAll}[4]{
\renewcommand{\ps@myheadings}{
\renewcommand{\@oddhead}{{\scriptsize #1 \hfil #2}}
\renewcommand{\@evenhead}{\@oddhead}
\renewcommand{\@evenfoot}{{\scriptsize #3}\hfil
        \textrm{\thepage}\hfil{\scriptsize #4}}
\renewcommand{\@oddfoot}{\@evenfoot}}
}

\def\NOW{\TODAY;\timenow}

\newcommand{\DRAFT}{
\renewcommand{\@evenhead}{\hfil DRAFT \hfil}
\renewcommand{\@oddhead}{\@evenhead}
}

\newcommand{\NowFootNum}{
\renewcommand{\@evenfoot}{{\scriptsize \jobname.tex}\hfil
        \textrm{\thepage}\hfil {\scriptsize \signature\ \NOW}}
\renewcommand{\@oddfoot}{\@evenfoot}
}

\newcommand{\NowFoot}{
\renewcommand{\@evenfoot}{{\scriptsize \signature}\hfil {\scriptsize \NOW}}
\renewcommand{\@oddfoot}{\@evenfoot}
}


\def\fixNumberingInArticle{
\@addtoreset{figure}{section} \@addtoreset{equation}{section}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
}

\def\fixNumberingInAppendix{
\setcounter{section}{0}
\renewcommand{\theequation}{\Alph{section}.\arabic{equation}}
\renewcommand{\thesection}{\Alph{section}}
\setcounter{equation}{0} }


\makeatother


\newcommand{\doubleDense}{
\setlength{\oddsidemargin}{0mm} \setlength{\evensidemargin}{0mm}
\addtolength{\textheight}{55mm} \addtolength{\textwidth}{43mm}
\setlength{\topmargin}{0mm} \setlength{\headsep}{4mm} \voffset=-20mm
\hoffset=-20mm \columnseprule=.01pt }

